Fine-tuning can Help Detect Pretraining Data from Large Language Models

In the era of large language models (LLMs), detecting pretraining data has been increasingly important due to concerns about fair evaluation and ethical risks. Current methods differentiate members and non-members by designing scoring functions, like Perplexity and Min-k%. However, the diversity and complexity of training data magnifies the difficulty of distinguishing, leading to suboptimal performance in detecting pretraining data. In this paper, we first explore the benefits of unseen data, which can be easily collected after the release of the LLM. We find that the perplexities of LLMs shift differently for members and non-members, after fine-tuning with a small amount of previously unseen data. In light of this, we introduce a novel and effective method termed Fine-tuned Score Deviation(FSD), which improves the performance of current scoring functions for pretraining data detection. In particular, we propose to measure the deviation distance of current scores after fine-tuning on a small amount of unseen data within the same domain. In effect, using a few unseen data can largely decrease the scores of all non-members, leading to a larger deviation distance than members. Extensive experiments demonstrate the effectiveness of our method, significantly improving the AUC score on common benchmark datasets across various models.

==> src/5_relatedWork.tex <==
\section{RELATED WORK}
Pretraining data detection, which is an increasingly important topic for large language models, relates to a large amount of literature on membership inference attacks and data contamination. We discuss some of the relevant works to ours in two directions below.

\paragraph{Membership Inference Attacks}
Our work mainly studies how to detect a given example in the pretraining data, which is consistent with the objective of membership inference attacks (MIAs)~\citep{shokri2017membership, truex2019demystifying}. This task aims to determine whether a given data point is a member of training data. Metric-based attack methods, such as loss~\citep{yeom2018privacy}, entropy~\citep{salem2019ml}, confidence~\citep{liu2019socinf} and gradient~\citep{liu2023gradient}, infer membership of data by comparing the calculated metric value with a preset threshold. Previous works have generalized metric-based methods to large language models~\citep{duan2024membership, xie2024recall, zhang2024min, mattern2023membership}, by calculating the based-likelihood metric (e.g., perplexity) for membership inference. Recent works apply MIAs to pretraining data detection by designing likelihood-based scoring functions to measure the membership of data~\citep{shidetecting, ye2024data}. In this work, we analyze the limitations of existing scoring functions for pretraining data detection, and design an effective method to improve their performance. In particular, this work is the first to explore the importance of collecting unseen data in pretraining data detection.
% As is shown in Table~\ref{auc_1}, our FSD achieves strong performance in pertaining data detection and is applicable to existing scoring functions in practical settings.

\paragraph{Data Contamination}
Data contamination has been studied in the literature~\citep{xu2024benchmark, magar2022data, balloccu2024leak}, where training data may inadvertently include evaluation benchmark data, resulting in unauthentic evaluation results. Thus, it is important to assess the leakage of benchmark data into pretraining data~\citep{zhou2023don}. On the one hand, model developers can remove evaluation benchmark data from training data by retrieval-based methods with access to pertaining data~\citep{ravaut2024much, chowdhery2023palm}. Specifically, those methods employ n-gram tokenization and string-matching for detecting data contamination~\citep{brown2020language, touvron2023llama2, team2023gemini, radford2019language}. On the other hand, researchers utilize prompting techniques~\citep{ golchintime}, performance analysis~\citep{ye2024data, debenedetti2024privacy}, model likelihood~\citep{orenproving, shidetecting, xu2024benchmarking} to detect potential contamination without access to the training data. Our work focuses on pretraining data detection, an area that is similar to data contamination. Different from data contamination detection, our FSD can also be applied to the  detection of copyrighted resources in real-world scenarios.

%Different from the above literature that focuses on classification tasks, we mainly consider a training-free solution to improve noise-robust ICL for generation tasks
%method can be also applied to detect benchmark data among data contamination.

% Our work focuses on the application of MIA to pretraining data detection, an area that has received limited attention in previous research efforts.


==> table/expe_auc_2.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{AUC score for detecting pretraining examples from the various models on arXivTection for our method and baselines. \textit{Pre.} and \textit{Fine.} denote the baseline methods and our method, respectively. \textbf{Bold} shows the best AUC within each column. 
} \label{auc_2}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{GPT-J-6B}} & \multicolumn{2}{c}{\textbf{OPT-6.7B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{LLaMA-7B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Method} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.}\\
\midrule

Perplexity & 0.79 & \textbf{0.96} & 0.68 & \textbf{0.89} & 0.77 & \textbf{0.95} & 0.68 & \textbf{0.92} & 0.79 & \textbf{0.95} \\
Lowercase & 0.59 & \textbf{0.81} & 0.58 & \textbf{0.70} & 0.60 & \textbf{0.77} & 0.50 & \textbf{0.69} & 0.62 & \textbf{0.75} \\
Zlib & 0.64 & \textbf{0.96} & 0.55 & \textbf{0.89} & 0.63 & \textbf{0.95} & 0.57 & \textbf{0.91} & 0.65 & \textbf{0.95} \\
\textsc{Min-k\% Prob} & 0.85 & \textbf{0.92} & 0.74 & \textbf{0.84} & 0.84 & \textbf{0.91} & 0.76 & \textbf{0.86} & 0.85 & \textbf{0.91} \\

\bottomrule
\end{tabular}
\end{table*}





==> table/expe_book.tex <==
% \begin{table*}[ht]
% \centering
% \footnotesize
% %\caption{Accuracy score for copyrighted book detection with baselines and our method from LLaMA-7B on BookMIA and BookTection. \textit{Pre.} and \textit{Fine.} respectively denote the baseline methods and our method. 
%\textbf{Bold} shows the superior result.} 
% minipage
\label{book_acc}
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{BookMIA}} & \multicolumn{2}{c}{\textbf{BookTection}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
% & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} \\
% \midrule

% Perplexity & 66.9 & \textbf{85.4} & 59.0 & \textbf{96.5} \\
% Lowercase & 64.5 & \textbf{73.0} & 67.0 & \textbf{69.2} \\
% Zlib & 65.3 & \textbf{86.4} & 57.4 & \textbf{98.6} \\
% \textsc{Min-k\%} & 68.1 & \textbf{82.1} & 59.5 & \textbf{93.9} \\

% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table}[h]
    \centering
    \begin{minipage}{.5\linewidth}
        \centering
        \footnotesize
        \caption{Accuracy score for copyrighted book detection with baselines and our method from LLaMA-7B on BookMIA and BookTection.}
        \label{book_acc}
        \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{BookMIA}} & \multicolumn{2}{c}{\textbf{BookTection}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} \\
        \midrule
        
        Perplexity & 66.9 & \textbf{85.4} & 59.0 & \textbf{96.5} \\
        Lowercase & 64.5 & \textbf{73.0} & 67.0 & \textbf{69.2} \\
        Zlib & 65.3 & \textbf{86.4} & 57.4 & \textbf{98.6} \\
        \textsc{Min-k\%} & 68.1 & \textbf{82.1} & 59.5 & \textbf{93.9} \\
        \bottomrule
        \end{tabular}
    \end{minipage}%
    \hspace{0.02\linewidth} % 调整两个表格之间的间距
    \begin{minipage}{.45\linewidth}
        \centering
        \footnotesize
        \caption{AUC score for copyrighted book detection with baselines and our method from LLaMA-7B on BookMIA and BookTection.}
        \label{book_auc}
        \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{BookMIA}} & \multicolumn{2}{c}{\textbf{BookTection}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} \\
        \midrule
        
        Perplexity & 0.710 & \textbf{0.910} & 0.564 & \textbf{0.995} \\
        Lowercase & 0.664 & \textbf{0.770} & 0.708 & \textbf{0.779} \\
        Zlib & 0.568 & \textbf{0.920} & 0.474 & \textbf{0.999} \\
        \textsc{Min-k\%} & 0.716 & \textbf{0.880} & 0.587 & \textbf{0.979} \\

        \bottomrule
        \end{tabular}
    \end{minipage}
\end{table}

==> table/expe_fpr_2.tex <==
\begin{table*}[!ht]
\centering
\footnotesize
\caption{TPR@5\%FPR for detecting pretraining examples from the given model on arXivTection for and baselines. \textit{Pre.} and \textit{Fine.} denote the baseline methods and our method, respectively. \textbf{Bold} shows the best TPR within each column. 
} \label{fpr_2}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{GPT-J-6B}} & \multicolumn{2}{c}{\textbf{OPT-6.7B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{LLaMA-7B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Method} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} & \textit{Pre.} & \textit{Fine.} \\
\midrule

Perplexity & 0.26 & \textbf{0.79} & 0.12 & \textbf{0.63} & 0.25 & \textbf{0.66} & 0.10 & \textbf{0.81} & 0.27 & \textbf{0.77} \\
Lowercase & 0.13 & \textbf{0.23} & 0.15 & \textbf{0.22} & 0.15 & \textbf{0.25} & 0.09 & \textbf{0.16} & 0.13 & \textbf{0.20} \\
Zlib & 0.15 & \textbf{0.80} & 0.07 & \textbf{0.60} & 0.14 & \textbf{0.50} & 0.08 & \textbf{0.66} & 0.16 & \textbf{0.77} \\
\textsc{Min-k\%} & 0.42 & \textbf{0.57} & 0.24 & \textbf{0.45} & 0.41 & \textbf{0.35} & 0.24 & \textbf{0.45} & 0.40 & \textbf{0.58} \\

 
\bottomrule
\end{tabular}
\end{table*}








==> table/expe_time_auc.tex <==
% \begin{table*}[t]
% \centering
% \footnotesize
% \caption{AUC score for detecting pretraining examples from the LLaMA-7B model with our method and baselines. \textit{Base} and \textit{\textbf{+Ours}} denote the baseline methods and our method, respectively. \textbf{Bold} shows the superior result. 
% } \label{time_auc}
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{WikiMIA}} & \multicolumn{2}{c}{\textbf{Deletion}} & \multicolumn{2}{c}{\textbf{Replacement}} \\
% \cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
% & \textit{Base} & \textit{\textbf{+Ours}} & \textit{Base} & \textit{\textbf{+Ours}} & \textit{Base} & \textit{\textbf{+Ours}} \\
% \midrule

% Perplexity & 0.64 &\textbf{0.92} & 0.62 & \textbf{0.76} & 0.54 & \textbf{0.71} \\
% Lowercase & 0.58 &\textbf{0.69} & 0.58 & \textbf{0.62} & 0.52 & \textbf{0.63} \\
% Zlib & 0.62 & \textbf{0.90} & 0.58 & \textbf{0.72} & 0.55 & \textbf{0.68} \\
% \textsc{Min-k\%} & 0.65 & \textbf{0.85} & 0.61 & \textbf{0.69} & 0.54 & \textbf{0.67} \\

% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\footnotesize
\caption{AUC score for detecting pretraining examples from the LLaMA-7B model with our method and baselines. \textit{Base} and \textit{\textbf{+Ours}} denote the baseline methods and our method, respectively. \textbf{Bold} shows the superior result. 
} \label{time_auc}
\begin{tabular}{lcccccc}
\toprule
\multirow{1}{*}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{WikiMIA}} & \multicolumn{1}{c}{\textbf{Deletion}} & \multicolumn{1}{c}{\textbf{Replacement}} \\

\midrule

Perplexity & 0.64/ \textbf{0.92} & 0.62/ \textbf{0.76} & 0.54/ \textbf{0.71} \\
Lowercase & 0.58/ \textbf{0.69} & 0.58/ \textbf{0.62} & 0.52/ \textbf{0.63} \\
Zlib & 0.62/ \textbf{0.90} & 0.58/ \textbf{0.72} & 0.55/ \textbf{0.68} \\
\textsc{Min-k\%} & 0.65/\textbf{0.85} & 0.61/ \textbf{0.69} & 0.54/ \textbf{0.67} \\

\bottomrule
\end{tabular}
\end{table*}


==> table/expe_time_replace.tex <==
\begin{table}[h!]
\centering
\caption{An illustration of timestamp differences between the member and non-member distributions.}
\begin{tabular}{p{6cm} p{6cm}}
\toprule
\multicolumn{1}{c}{\textbf{Members}} & \multicolumn{1}{c}{\textbf{Non-Members}}\\ 
\midrule
The \textcolor{red}{2023} On 30 June or 2 July \textcolor{red}{2023}, the Armed Forces of the Democratic Republic of the Congo and United Nations forces launched an offensive against rebel groups in the Masisi and Walikale.
& The 95th Academy Awards was a ceremony held by the Academy of Motion Picture Arts and Sciences (AMPAS) on March 12, \textcolor{blue}{2023}, at the Dolby Theatre in Los Angeles. \\
\midrule
In \textcolor{red}{2023}, a series of groundbreaking diplomatic meetings was held between Wang Yu-chi, in his official capacity as the Minister of the Mainland Affairs Council (MAC) of the Republic of China (ROC).
& The 36th Annual Nickelodeon Kids' Choice Awards ceremony was held on March 4, \textcolor{blue}{2023}, at the Microsoft Theater in Los Angeles, California with Nate Burleson and Charli D'Amelio. \\
\midrule
Concluding observations on the second periodic report of the Holy See was a \textcolor{red}{2023} report issued by the Office of the United Nations High Commissioner for Human Rights.
& The \textcolor{blue}{2023} Summer Metro Manila Film Festival is an ongoing iteration of the annual Summer Metro Manila Film Festival held in Metro Manila and throughout the Philippines.\\
\midrule
The 2023 European Aquatics Championships took place from 13 to 24 August \textcolor{red}{2023} in Berlin, Germany.
& On February 11, \textcolor{blue}{2023}, an octagonal unidentified flying object was detected over northern Montana. \\
\midrule
The centenary of the outbreak of World War I was commemorated in Europe in late July and early August \textcolor{red}{2023}.W
& The \textcolor{blue}{2023} Tokyo Marathon was the 16th edition of the annual marathon race in Tokyo, held on Sunday, 5 March \textcolor{blue}{2023}. \\
\bottomrule
\end{tabular}
\label{timestamp}
\end{table}


==> table/expe_trainSize_auc.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{AUC score for pretraining data detection from LLaMA-7B model on WikiMIA. \textbf{Sampling ratio} denotes that sampling data using varying sampling ratios. Notably, the ratio of 0 denotes baseline methods. \textbf{Bold} shows the superior result.
} 
\label{split_auc}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Sampling ratio}} \\
\cmidrule(lr){2-11}
\textbf{Method}&0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 \\
\midrule

Perplexity & 0.65 & 0.86 & 0.88 & 0.92 & 0.93 & 0.95 & 0.95 & 0.96 & 0.96 & \textbf{0.98} \\
Lowercase & 0.58 & 0.60  & 0.62 & 0.69 & 0.75 & 0.80 & 0.80 & 0.83 & 0.87 & \textbf{0.88} \\
Zlib & 0.61 & 0.82 & 0.88 & 0.90 & 0.93 & 0.95 & 0.95 & 0.95 & 0.97 & \textbf{0.98} \\
\textsc{Min-k\%} & 0.66 & 0.77 & 0.82 & 0.86 & 0.86 & 0.90 & 0.92 & 0.93 & 0.95 & \textbf{0.96} \\

\bottomrule
\end{tabular}
\end{table*}

==> table/expe_trainSize_fpr.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{TPR@5\%FPR socre for pretraining data detection from LLaMA-7B model on WikiMIA. \textbf{Sampling
ratio} denotes that sampling data using varying sampling ratios. Notably, the ratio of 0 denotes
baseline methods. \textbf{Bold} shows the superior result. 
} 
\label{trainsize_fpr}
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{9}{c}{\textbf{Sampling ratio}} \\
\cmidrule(lr){2-11}
\textbf{Method} & 0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 \\
\midrule

Perplexity & 0.11 & 0.26 & 0.22 & 0.44 & 0.56 & 0.67 & 0.72 & 0.64 & 0.68 & 0.98 \\
Lowercase & 0.08 & 0.10 & 0.12 & 0.17 & 0.22 & 0.30 & 0.30 & 0.39 & 0.29 & 0.57 \\
Zlib & 0.10 &0.24& 0.28 & 0.46 & 0.52 & 0.70 & 0.67 & 0.61 & 0.78 & 0.98 \\
\textsc{Min-k\% Prob} & 0.16 & 0.13 & 0.18 & 0.28 & 0.21 & 0.42 & 0.46 & 0.52 & 0.51 & 0.61 \\

\bottomrule
\end{tabular}
\end{table*}
